BIoTA Control-Aware Attack Analytics for Building Internet of Things

Modern building control systems adopt demand control heating, ventilation, and cooling (HVAC) for increased energy efficiency. The integration of the Internet of Things (IoT) in the building control system can determine real-time demand, which has made the buildings smarter, reliable, and efficient. As occupants in a building are the main source of continuous heat and $CO_2$ generation, estimating the accurate number of people in real-time using building IoT (BIoT) system facilities is essential for optimal energy consumption and occupants' comfort. However, the incorporation of less secured IoT sensor nodes and open communication network in the building control system eventually increases the number of vulnerable points to be compromised. Exploiting these vulnerabilities, attackers can manipulate the controller with false sensor measurements and disrupt the system's consistency. The attackers with the knowledge of overall system topology and control logics can launch attacks without alarming the system. This paper proposes a building internet of things analyzer (BIoTA) framework\footnote{https://github.com/imtiazulhaque/research-implementations/tree/main/biota} that assesses the smart building HVAC control system's security using formal attack modeling. We evaluate the proposed attack analyzer's effectiveness on the commercial occupancy dataset (COD) and the KTH live-in lab dataset. To the best of our knowledge, this is the first research attempt to formally model a BIoT-based HVAC control system and perform an attack analysis.

==> sections/Implementation.tex <==
\section{Implementation} \label{Sec:setup_env}
The implementation source code for BIoTA framework is available in GitHub~\cite{biota2020}.
We use the satisfiability modulo theory (SMT) to solve and optimize a set of constraints that uses efficient, logical ideas ~\cite{barrett2018satisfiability}. We encode the conditions using integer and real terms. Based on the satisfiability,  the model produces SAT or UNSAT results. The SAT result outputs an attack vector, the complete information of sensor measurement alteration for launching a successful attack on the BIoT. The formal threat modeling has been implemented using Z3 library~\cite{de2008z3}. We have used python API of Z3 SMT solver for both solving and optimizing our modeling constraints. The psypy library is used to calculate and extract necessary psychrometric parameters from temperature and relative humidity~\cite{psypy2020}. The implementation of the library follows ASHRAE standard. A Dell Precision 7920 Tower workstation with Intel Xeon Silver 4110 CPU @3.0GHz, 32 GB memory, 4 GB NVIDIA Quadro P1000 GPU is used to run these experiments.
